Pileup and Underlying Event Mitigation with Iterative Constituent Subtraction

The hard-scatter processes in hadronic collisions are often largely contaminated with soft background coming from pileup in proton-proton collisions, or underlying event in heavy-ion collisions. This paper presents a new background subtraction method for jets and event observables (such as missing transverse energy) which is based on the previously published Constituent Subtraction algorithm. The new subtraction method, called Iterative Constituent Subtraction, applies event-wide implementation of Constituent Subtraction iteratively in order to fully equilibrate the background subtraction across the entire event. Besides documenting the new method, we provide guidelines for setting the free parameters of the subtraction algorithm. Using particle-level simulation, we provide a comparison of Iterative Constituent Subtraction with several existing methods from which we conclude that the new method has a significant potential to improve the background mitigation in both proton-proton and heavy-ion collisions.

==> Makefile <==
LATEX    = latex
BIBTEX   = bibtex
DVIPS    = dvips

BASENAME = ms

default: dopdflatexwithbibtex


dopdflatex:
	pdflatex  ${BASENAME}
	pdflatex  ${BASENAME}
	make clean

dopdflatexwithbibtex:
	pdflatex  ${BASENAME}
	pdflatex  ${BASENAME}
	bibtex    ${BASENAME}
	pdflatex  ${BASENAME}
	pdflatex  ${BASENAME}
	make clean


clean:
	rm -f *.aux *.log *.blg *.brf *.cb *.ind *.idx *.ilg  \
	      *.inx *.dvi *.toc *.out *~  spellTmp ${BASENAME}.ps



==> defs.tex <==
%
% User-defined latex commands
%

\RequirePackage{xspace}

\newcommand{\tev}               {\ensuremath{~\mathrm{TeV}}\xspace}
\newcommand{\gev}               {\ensuremath{~\mathrm{GeV}}\xspace}
\newcommand{\mev}               {\ensuremath{~\mathrm{MeV}}\xspace}

% Jet mass related
\newcommand{\mjet}               {\ensuremath{m^{\rm jet}}\xspace}
\newcommand{\mlead}              {\ensuremath{\mjet_{1}}\xspace}
\newcommand{\mleadavg}           {\ensuremath{\langle\mlead\rangle}\xspace}
\newcommand{\Mjet}               {\ensuremath{m^{\rm jet}}\xspace}
\newcommand{\massjet}            {\mjet}
\newcommand{\mjetAvg}            {\ensuremath{\langle\mjet\rangle}\xspace}
\newcommand{\masstrkjet}         {\ensuremath{m^{\rm track \; jet}}\xspace}

% Particle (and mass) related
\newcommand{\Wmass}              {\ensuremath{m_{\Wboson}}\xspace}
\newcommand{\WmassT}             {\ensuremath{m^{\Wboson}_{\rm T}}\xspace}
\newcommand{\topmass}            {\ensuremath{m_{t}}\xspace}
\newcommand{\mTransv}            {\ensuremath{m_{\rm T}}\xspace}
\newcommand{\massZprime}         {\ensuremath{m_{\Zprime}}\xspace}

% Jet algorithm and grooming related
\newcommand{\antikt}             {anti-\ensuremath{k_{t}}\xspace}
\newcommand{\akt}                {\antikt\xspace}
\newcommand{\aktfour}            {\antikt \ensuremath{R=0.4}\xspace}
\newcommand{\aktten}            {\antikt \ensuremath{R=1.0}\xspace}
\newcommand{\kt}                 {\ensuremath{k_{t}}\xspace}
\newcommand{\ca}                 {Cambridge--Aachen\xspace}
\newcommand{\CamKt}              {\ensuremath{\mathrm{C/A}}\xspace}
\newcommand{\CASix}              {\CamKt, \ensuremath{R=0.6}\xspace}
\newcommand{\CAFat}              {\CamKt, \ensuremath{R=1.2}\xspace}
\newcommand{\CAPrune}            {\CamKt, \ensuremath{R=1.2} (pruned)\xspace}
\newcommand{\CAFilt}             {\CamKt, \ensuremath{R=1.2} (filtered)\xspace}
\newcommand{\SISCone}            {SISCone}
\newcommand{\SISConeSiz}         {\SISCone, \ensuremath{R=0.6}\xspace}
\newcommand{\minKt}              {\ensuremath{\min\left(\pti^2, \ptj^2\right)}\xspace}
\newcommand{\minAKt}             {\ensuremath{\min\left(\pti^{-2}, \ptj^{-2}\right)}\xspace}
\newcommand{\minGen}             {\ensuremath{\min\left(\pti^{2p}, \ptj^{2p}\right)}\xspace}
\newcommand{\pt}                 {\ensuremath{p_{\mathrm{T}}}\xspace}
\newcommand{\et}                 {\ensuremath{E_{\mathrm{T}}}\xspace}
\newcommand{\etmiss}             {\ensuremath{E_{\mathrm{T}}^{\mathrm{miss}}}\xspace}
\newcommand{\etmissx}            {\ensuremath{E_{\mathrm{T},x}^{\mathrm{miss}}}\xspace}
\newcommand{\etmissVec}          {\ensuremath{\vec{E}_{\mathrm{T}}^{\mathrm{miss}}}\xspace}
\newcommand{\pttrue}             {\ensuremath{\pt^{\mathrm{true}}}\xspace}
\newcommand{\ptreco}             {\ensuremath{\pt^{\mathrm{reco}}}\xspace}
\newcommand{\Rij}                {\ensuremath{R_{ij}}\xspace}
\newcommand{\DRij}               {\ensuremath{\Delta\Rij}\xspace}
\newcommand{\DRratio}            {\ensuremath{\frac{(\DRij)^2}{R^2}}\xspace}
\newcommand{\sjone}              {\ensuremath{j_{1}}\xspace}
\newcommand{\sjtwo}              {\ensuremath{j_{2}}\xspace}
\newcommand{\msubjone}           {\ensuremath{m^{\sjone}}\xspace}
\newcommand{\msubjtwo}           {\ensuremath{m^{\sjtwo}}\xspace}
\newcommand{\ptsubjone}          {\ensuremath{\pt^{\sjone}}\xspace}
\newcommand{\ptsubjtwo}          {\ensuremath{\pt^{\sjtwo}}\xspace}
\newcommand{\Rsubjets}           {\ensuremath{R_{\sjone,\sjtwo}}\xspace}
\newcommand{\DRsubjets}          {\ensuremath{\Delta\Rsubjets}\xspace}
\newcommand{\Nsubjet}            {\ensuremath{N_{\rm subjet}}\xspace}
\newcommand{\pti}                {\ensuremath{p_{\mathrm{T},i}}\xspace}
\newcommand{\pticorr}            {\ensuremath{\pti^{\rm corr}}\xspace}
\newcommand{\ptpatch}            {\ensuremath{p_{{\rm T patch}}}\xspace}
\newcommand{\ptj}                {\ensuremath{p_{{\rm T}j}}\xspace}
\newcommand{\phii}               {\ensuremath{\phi_{i}}\xspace}
\newcommand{\yi}                 {\ensuremath{y_{i}}\xspace}
\newcommand{\mi}                 {\ensuremath{m_{i}}\xspace}
\newcommand{\mdelta}             {\ensuremath{m_{\delta}}\xspace}
\newcommand{\mdeltai}            {\ensuremath{m_{\delta i}}\xspace}
\newcommand{\mdeltapatch}        {\ensuremath{m_{\delta \rm patch}}\xspace}
\newcommand{\mdeltaicorr}        {\ensuremath{\mdeltai^{\rm corr}}\xspace}
\newcommand{\ycut}               {\ensuremath{y_{\rm cut}}\xspace}
\newcommand{\mcut}               {\ensuremath{m_{\rm cut}}\xspace}
\newcommand{\ymin}               {\ensuremath{y_{\min}}\xspace}
\newcommand{\fcut}               {\ensuremath{f_{\rm cut}}\xspace}
\newcommand{\Rsub}               {\ensuremath{R_{\rm sub}}\xspace}
\newcommand{\drsub}              {\ensuremath{\Rsub}\xspace}
\newcommand{\mufrac}             {\ensuremath{\mu_{\rm frac}}\xspace}
\newcommand{\rcut}               {\ensuremath{R_{\rm cut}}\xspace}
\newcommand{\zcut}               {\ensuremath{z_{\rm cut}}\xspace}
\newcommand{\largeR}             {large-\ensuremath{R}\xspace}
\newcommand{\LargeR}             {Large-\ensuremath{R}\xspace}


% Jet substructure related
\newcommand{\shapeV}             {\ensuremath{{\cal V}}\xspace}
\newcommand{\htt}                {HEPTopTagger\xspace}
\newcommand{\subjetpt}           {\ensuremath{\pT^{\rm subjet}}\xspace}
\newcommand{\subjetptl}          {\ensuremath{\pT^{\rm subjet, lead}}\xspace}
\newcommand{\subjetptsl}         {\ensuremath{\pT^{\rm subjet, sublead}}\xspace}
\newcommand{\yij}                {\ensuremath{y_{ij}}\xspace}
\newcommand{\dcut}               {\ensuremath{d_{\rm cut}}\xspace}
\newcommand{\dmin}               {\ensuremath{d_{\min}}\xspace}
\newcommand{\dij}                {\ensuremath{d_{ij}}\xspace}
\newcommand{\Dij}                {\ensuremath{\sqrt{\dij}}\xspace}
\newcommand{\DOneTwo}            {\ensuremath{\sqrt{d_{12}}}\xspace}
\newcommand{\DTwoThr}            {\ensuremath{\sqrt{d_{23}}}\xspace}
\newcommand{\xj}                 {\ensuremath{x_{J}}\xspace}
\newcommand{\jetFunc}            {\ensuremath{J^{(eik),c} (\mjet, \pT, R)}\xspace}
\newcommand{\tauN}               {\ensuremath{\tau_N}\xspace}
\newcommand{\tauOne}             {\ensuremath{\tau_{1}}\xspace}
\newcommand{\tauTwo}             {\ensuremath{\tau_{2}}\xspace}
\newcommand{\tauThr}             {\ensuremath{\tau_{3}}\xspace}
\newcommand{\tauTwoOne}          {\ensuremath{\tau_{21}}\xspace}
\newcommand{\tauThrTwo}          {\ensuremath{\tau_{32}}\xspace}
\newcommand{\COneThr}            {\ensuremath{C_{1}^{(3)}}\xspace}

% Samples
\newcommand{\Zprimett}           {\ensuremath{Z'\ra t\bar{t}}\xspace}
\newcommand{\Zprime}             {\ensuremath{Z'}\xspace}
\newcommand{\Zqq}                {\ensuremath{Z\ra q\bar{q}}\xspace}
\newcommand{\Wqq}                {\ensuremath{W\ra q\bar{q}}\xspace}


% terminology
\newcommand{\mpi}                {multiple parton interactions\xspace}
\newcommand{\fourvector}         {4-vector\xspace}
\newcommand{\fourmomentum}       {4-momentum\xspace}
\newcommand{\fourmomenta}        {4-momenta\xspace}
\newcommand{\pileup}             {pileup\xspace}
\newcommand{\Pileup}             {Pileup\xspace}
\newcommand{\areaSubtraction}    {Area Subtraction\xspace}
\newcommand{\subtraction}        {Constituent Subtraction\xspace}
\newcommand{\ics}                {Iterative Constituent Subtraction\xspace}



       
\newcommand{\avg}[1]             {\left< #1 \right>} % for e.g. <\mu>

\newcommand{\rhom}               {\ensuremath{\rho_{m}}\xspace}

\newcommand{\Rmin}               {\ensuremath{R_{\rm min}}}
\newcommand{\DeltaR}             {\ensuremath{\Delta R}\xspace}
\newcommand{\DeltaRhard}         {\ensuremath{\Delta R^{\mathrm{hard}}}\xspace}
\newcommand{\DeltaRmax}          {\ensuremath{\Delta R^{\mathrm{max}}}\xspace}
\newcommand{\DeltaRik}           {\ensuremath{\Delta R_{i,k}}\xspace}
\newcommand{\Dik}                {\ensuremath{D_{i,k}}\xspace}
\newcommand{\Dy}                 {\ensuremath{\Delta y}\xspace}
\newcommand{\Deta}               {\ensuremath{\Delta\eta}\xspace}
\newcommand{\Dphi}               {\ensuremath{\Delta\phi}\xspace}
\newcommand{\maxEta}             {\ensuremath{\eta^{\mathrm{max}}}\xspace}


% pileup subtraction related
\newcommand{\ptInput}            {\ensuremath{\pt^{\mathrm{input}}}\xspace}
\newcommand{\ptOutput}           {\ensuremath{\pt^{\mathrm{output}}}\xspace}
\newcommand{\ghostpt}            {\ensuremath{\pt^g}\xspace}
\newcommand{\ghostptk}           {\ensuremath{p_{{\rm T}k}^g}\xspace}
\newcommand{\ghostptkSquared}    {\ensuremath{p_{{\rm T}k}^{g2}}\xspace}
\newcommand{\ghostphik}          {\ensuremath{\phi_{k}^g}\xspace}
\newcommand{\ghostyk}            {\ensuremath{y_{k}^g}\xspace}
\newcommand{\ghostm}             {\ensuremath{m^g}\xspace}
\newcommand{\ghostmk}            {\ensuremath{m_{k}^g}\xspace}
\newcommand{\ghostmkSquared}     {\ensuremath{m_{k}^{g2}}\xspace}
\newcommand{\ghostmdelta}        {\ensuremath{m_{\delta}^g}\xspace}
\newcommand{\ghostmdeltak}       {\ensuremath{m_{\delta k}^g}\xspace}
\newcommand{\ghostptavg}         {\ensuremath{\langle\ghostpt\rangle}\xspace}
\newcommand{\ghostfm}            {\ensuremath{g_{\mu}}\xspace}
\newcommand{\ghostfmi}           {\ensuremath{g_{\mu,i}}\xspace}
\newcommand{\ghostdensity}       {\ensuremath{\nu_{g}}\xspace}
\newcommand{\ghostrho}           {\ensuremath{\ghostdensity\ghostptavg}\xspace}
\newcommand{\Aghost}             {\ensuremath{A_{g}}\xspace}
\newcommand{\Amu}                {\ensuremath{A_{\mu}}}
\newcommand{\Amui}               {\ensuremath{A_{\mu, i}}}
\newcommand{\jetarea}            {\ensuremath{A^{\mathrm{jet}}}\xspace}
\newcommand{\jetareafm}          {\ensuremath{A^{\mathrm{jet}}_{\mu}}\xspace}
\newcommand{\jetareai}           {\ensuremath{\jetarea_{i}}\xspace}
\newcommand{\areapatch}          {\ensuremath{A_{\rm patch}}\xspace}
\newcommand{\rkt}                {\ensuremath{R_{\kt}}\xspace}
\newcommand{\yphi}                {\ensuremath{y -\phi}\xspace}
\newcommand{\etaphi}                {\ensuremath{\eta -\phi}\xspace}

\newcommand{\ptorig}             {\ensuremath{p_T^{\rm orig}}\xspace}
\newcommand{\npu}                {\ensuremath{N_{PU}}\xspace}
\newcommand{\avgnpu}             {\ensuremath{\avg{\npu}}\xspace}
\newcommand{\avgrho}             {\ensuremath{\avg{\rho}}\xspace}
\newcommand{\sigmarho}           {\ensuremath{\sigma[\rho]}\xspace}
\newcommand{\Niter}           {\ensuremath{N^{\mathrm{iter}}}\xspace}



\newcommand{\meanDelta}          {\ensuremath{\langle \Delta x \rangle}\xspace}
\newcommand{\sigmaDelta}         {\ensuremath{\sigma[\Delta x]}\xspace}
\newcommand{\ptSum}         {\ensuremath{\langle\sum \pt\rangle}\xspace}
\newcommand{\ptSumTrue}         {\ensuremath{\langle\sum \pt^{\mathrm{true}}\rangle}\xspace}

